Self-Attention Linguistic-Acoustic Decoder

The conversion from text to speech relies on the accurate mapping from linguistic to acoustic symbol sequences, for which current practice employs recurrent statistical models like recurrent neural networks. Despite the good performance of such models (in terms of low distortion in the generated speech), their recursive structure tends to make them slow to train and to sample from. In this work, we try to overcome the limitations of recursive structure by using a module based on the transformer decoder network, designed without recurrent connections but emulating them with attention and positioning codes. Our results show that the proposed decoder network is competitive in terms of distortion when compared to a recurrent baseline, whilst being significantly faster in terms of CPU inference time. On average, it increases Mel cepstral distortion between 0.1 and 0.3 dB, but it is over an order of magnitude faster on average. Fast inference is important for the deployment of speech synthesis systems on devices with restricted resources, like mobile phones or embedded systems, where speaking virtual assistants are gaining importance.

==> results.tex <==

\section{Experimental Setup}
\label{sec:experiments}


\subsection{Dataset}

The experiments are performed with a professional male speaker from the TCSTAR~\cite{bonafonte2006tc} dataset, thus with recording studio quality. We have 7.5 hours of speech from this speaker, which are divided in $80\%$ for training, $10\%$ for validation and $10\%$ for test. 

\subsection{Neural Vocoder Architecture Setup}
Several experiments with the unconditioned SampleRNN have been done to define the architecture and the optimizer parameters to be used in the remaining experiments in our TTS system. 
All experiments are conducted with a batch size of 128 sequences of length 1040. 

As shown in figure~\ref{fig:framernn}, the selected architecture has three tiers. The higher tier is composed of 2 GRU layers. The input is 80 samples (5 ms. at 16kHz) and the output is the condition to the mid tier. The conditioner is expanded into 5 conditioning vectors through a 1D convolutional layer. The mid tier is also composed of 2 GRU layers. In this case the input is formed by 16 samples in addition to the previous conditioning vector. Finally, the lowest tier contains a MLP with one hidden layer. Owing to the fact that SampleRNN predicts discrete categories corresponding to quantized sample values at 8 bits, we have an output layer of 256 units. Note that all recurrent and fully connected layers contain 1024 units.

\begin{figure}[!htpb]
     \centering
     \includegraphics[width=0.5\textwidth]{figures/framernn.pdf}
      \caption{Structure of the first two tiers of the system, with two RNN of 1024 hidden units. , a $FS=[20 \quad 4]$ and an up-sampling ratio of $r=4$. In the first tier we have an entry of 80 real valued samples and an activated conditioner flag. Both the input and the conditioner pass through their respective 1D convolution layer, and these outputs are linearly added. This will be the entrance to the first GRU, which will store the hidden state $h(k)$ to use it in the next tier as a conditioner. Then the output goes through the transposed convolution, performing the process of upsampling.  Finally these output enters to the second frame-level. The input inp($k=2$) is conditioned under the previous stored memory in the upper tier, $h(k)_{t-1}$ state. From here is followed the same process as the previous tier. }
       \label{fig:framernn}
    
\end{figure}


The original SampleRNN used uniform quantization, so we decided to test the possible performance increase when we apply $\mu$-law transformation to reduce the quantization noise. Listening to the newly generated samples clearly show the advantage of the $\mu$-law transformed distribution over the raw one. 

\newpage
As a final remark, the proposed vocoder system was built on top of a publicly available implementation of sampleRNN\footnote{https://github.com/deepsound-project/samplernn-pytorch} in PyTorch~\cite{paszke2017automatic}.


\subsection{TTS System: MUSA and SampleRNN}
\label{sec:results:SamplewithMusa}

As we are focusing on the acoustic model, all the durations are forced to be the annotated ones in the ground truth. 

We want to test the performance of the coupling under three different configurations:
\begin{itemize}
\item Independent Neural Vocoder (INV). In this case SampleRNN is trained with the acoustic parameterization from original speech samples.
\item Independently-trained MUSA-based Neural Vocoder (IMNV). For each utterance in the training corpus, we infer the acoustic parameter with the MUSA prediction. These parameters are used as training samples for our neural vocoder replacing previous ground truth samples coming from the original speech samples.
\item Jointly-trained MUSA-based Neural Vocoder (JMNV). Same case as previous one but adding an additional training stage where the full joint model (MUSA+SampleRNN) is tuned end-to-end.
\end{itemize}






\subsection{Objective Evaluation}

We observe an abrupt behavior of the all losses after certain epochs. We believe that the learning rate could be too big after that epoch, thus we decide to decrease the learning rate monotonically with a scheduler. This decays the initial learning rate by a $\gamma$ factor every $E$ epochs. Specifically, we set up an initial learning rate (lr) of $0.001$ with $\gamma = 0.1$. This way we have:

\begin{equation}
    \left\{\begin{matrix}
 \textrm{lr} = 10^{-3}&  \text{epoch} < 15 \\ 
 \textrm{lr} = 10^{-4}&  15 \le \text{epoch} < 35\\ 
 \textrm{lr} = 10^{-5}&   \text{epoch} > 35 
\end{matrix}\right.
\end{equation}


In table~\ref{tbl:optim} we show the difference in test performance among three different optimizer executions. The test metric is the negative log-likelihood (NLL). These results confirm the effectiveness of the designed scheduler, being Adam the preferred option over RMSprop and so the one with which we combine the scheduler to obtain the best result.

\begin{table}[ht]
\caption{Comparison of the different tested optimizers in terms of the negative log-likelihood (NLL) (lower is better).}
\centering
\label{tbl:optim}
\begin{tabular}{c@{\hspace{1cm}}c}
\toprule
\textbf{Optimizer}  & \textbf{Average NLL Test} \\ \midrule
RMSprop             & 3.19                   \\
Adam                & 2.56             \\
Adam+Scheduler      & \textbf{2.41}             \\ \bottomrule
\end{tabular}
\end{table}

\begin{table}[!hbpt]
\caption{Comparison of SampleRNN test performance under different configurations in terms of the negative log-likelihood (NLL) (lower is better).}
\centering
\label{tbl:musasamplernn}
\begin{tabular}{c@{\hspace{1cm}}c}
\toprule
\textbf{Model Configuration}     & \textbf{Average NLL Test} \\ \midrule
INV  & 2.41\\
IMNV & 2.67\\
IMNV pre-trained & 2.66\\
JMNV & 2.47\\\bottomrule
\end{tabular}
\end{table}


As shown in the table~\ref{tbl:musasamplernn}, when we substitute the ground truth features (INV) with the ones predicted by MUSA (IMNV) there is a noticeable degradation in the test performance, as expected. We can slightly improve it by facilitating the convergence in a setup were IMNV is initialized with INV weights. Last row in the table shows how we can close the gap by tuning the joint structure (MUSA and SampleRNN) end-to-end. 


%\begin{figure}[ht]
%    \centering
    
%        \includegraphics[width=8cm]{figures/CONDMUSA/nopreMUSA.png}
%        \caption{nopreMUSA}
%%        \label{fig:nopreMUSA}
  
%\end{figure}



%\begin{figure}
 %   \centering
  %  \includegraphics[width=8cm]{figures/musaSampleRNN/MUSASamleRNN30.png}
   % \caption{NLL loss curve training jointly the two stage system}
    %\label{fig:MUSASampleRNN}
%\end{figure}


\subsection{Subjective Evaluation}
\label{sec:Subjres}



% \begin{table*}[!htpb]
% \caption{Subjective evaluation disaggregated results}
% \centering
% \begin{tabular}{@{}ccccc@{}}
% \toprule
% \begin{tabular}[c]{@{}c@{}}Musa+SampleRNN\\ (Joint Estimation)\end{tabular} & \begin{tabular}[c]{@{}c@{}}MUSA\\ (Baseline)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Musa+SampleRNN\\ (Pipeline)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Baseline OR\\ Joint Estimation\end{tabular} & \begin{tabular}[c]{@{}c@{}}Pipeline OR\\ Joint Estimation\end{tabular} \\ \midrule
% 36                                                                          & 15                                                        & 3                                                                   & 10                                                                    & 6                                                                     \\ \bottomrule
% \end{tabular}
% \label{tab:subj}
% \end{table*}



Objective tests performed well to compare different architectures and to suggest how well does the TTS work. But when analyzing the complete system, that is, the conditioned SampleRNN under the MUSA characteristics, we obtained similar results in all the performed experiments. To get a more in-depth evaluation of the model a subjective test is conducted to evaluate the naturalness of the TTS developed in this work and also to make a comparison with the baseline system, that is, Ahodecoder vocoder under MUSA parameterization.

A web based application was developed with the selected audio files obtained from the experiments, explained below, and volunteers were asked to rate the voices in a scale from one to five, one being bad and five being excellent. In the test each listener was asked to evaluate 5 sentences, randomly selected from the test set. In total 14 subjects took the test. 
The participants could listen the different recordings as many times as required to make comparisons between the different systems and select which system or systems produce the most natural speech. For every sentence, the listeners evaluated 3 different versions generated with the following 3 different systems:

\begin{itemize}
\item Baseline: using Ahodecoder to generate speech from the acoustic parameters predicted by MUSA~\cite{pascual2016deep} (MAHO)
\item Independently-trained MUSA-based Neural Vocoder (IMNV). 
\item Jointly-trained MUSA-based Neural Vocoder (JMNV). 
\end{itemize}


Table \ref{tab:subj} shows the results of the subjective test.  

\begin{table}[!htpb]
\caption{Preference test showing the best selected system or systems (in percentage).}
% 15 3 36 10 6

%21.4285714285714
%4.28571428571429
%51.4285714285714
%14.2857142857143
%8.57142857142857


\centering
\begin{tabular}{@{}ccccc@{}}\toprule
\shortstack{MAHO\\{~}} & \shortstack{IMNV\\{~}} & \shortstack{JMNV\\{~}} & \shortstack{JMNV OR\\MAHO} & \shortstack{JMNV\\IMNV}\\\midrule
21.4   &    4.3 &   51.4 & 14.3           & 8.6\\
\bottomrule
\end{tabular}
\label{tab:subj}
\end{table}


As it can be seen, independent training of MUSA and SampleRNN (IMNV) produces much worse results that the baseline system that uses the original decoder of Ahocoder (MAHO). MAHO is one of the preferred system in 50.0\% of the 70 evaluations, while IMNV is only one of the preferred systems in 12.9\% of the cases. However, the joint training of MUSA and SampleRNN effectively integrates both systems producing the best option. As we can see, JMNV is one of the systems in 74.3\% of the cases. 

The results IMNV are much worse than expected. An analysis of the result showed that there was a normalization problem that produced an inconsistency between MUSA prediction and the ground truth acoustic features. However, the results show that the joint training is able to overcome such limitation and is more robust to inconsistencies. 





%\toni{queda raro esto con una gráfica en apéndice. Entiendo que antes estaba aquí .. Si la quitas, imagino que por espacio, reescribe esto sin la figura. Sólo al final puedes poner que se muestra en apéndice, como inform. coplementaria. Pero de hecho, para ponerla allí, yo la borraría. No es lo que se pone en apend. Lo de histograma de ceps. si qué esta bien.

%Guardala para la presentación y ya está.}








